SearchGCN: Powering Embedding Retrieval by Graph Convolution Networks for E-Commerce Search

Graph convolution networks (GCN), which recently becomes new state-of-the-art method for graph node classification, recommendation and other applications, has not been successfully applied to industrial-scale search engine yet. In this proposal, we introduce our approach, namely SearchGCN, for embedding-based candidate retrieval in one of the largest e-commerce search engine in the world. Empirical studies demonstrate that SearchGCN learns better embedding representations than existing methods, especially for long tail queries and items. Thus, SearchGCN has been deployed into JD.com's search production since July 2020.

==> 2-relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Graph Convolution Network}
% origin, and laplacian smooth explanation
Neural networks that operate on graphs have previously been introduced in~\cite{gori2005} and~\cite{scarselli2009} as a form of recurrent neural network. Their frameworks apply propagation functions until node representations reach a stable fixed point. Later on, with the success of convolution neural networks in various domains, such as image classification~\cite{he2016}, semantic segmentation~\cite{jegou2017}, text classification~\cite{kim2014}, and machine translation~\cite{gehring2017},
there is an increasing interest in generalizing convolution network to graph domain. Advances in this Graph Convolution Network (GCN) directions are often categorized into spectral approaches and non-spectral approaches.

Spectral approaches work with a spectral representation of the graph. Originally, in the work of \citeauthor{bruna2013spectral}, the convolution operation is defined in the Fourier domain by computing the eigendecomposition of the graph Laplacian, which, however, requires intense computations. 
\citeauthor{kipf2016semi} alleviated the computational cost by developing an efficient layer-wise propagation rule based on a first-order approximation of spectral graph convolutions.
However, the layer-wise propagation rule still have two drawbacks during training procedure. First, the graph convolution requires full graph Laplacian, which is computational-expensive and even problematic for training with large graph. Second, the full graph Laplacian is computed from a fixed graph, which do not naturally generalize to unseen nodes. % TODO: kipf2016 model is able to work with large graph?

% graphSAGE, pinSAGE
The other non-spectral approaches define convolutions directly on the graph, by operating on a set of spatially close neighbors. GraphSAGE~\cite{hamilton2017inductive} avoided operating on the entire graph Laplacian by developing a learnable aggregation functions, which comprehensively scale the GCN algorithm to large graph and achieve the ability to generate node embeddings for previously unseen data. Additionally, the neighbor sampling in the work of GraphSAGE alleviate the computation cost to receptive fixed field during mini-batch training procedure. Later on, PinSAGE \cite{ying2018graph} scaled the GCN algorithm to the real item-item recommendation task with large graph having billions of nodes and edges, which paves the way of large-scale deep recommendation systems based on GCN architectures. 

% recent progress
Recently, there are plenty of GCN variants proved to be more effective than previous first wave of GCN exploration. LightGCN~\cite{he2020lightgcn} simplifies the GCN algorithm significantly by reducing the unnecessary and even noisy operations, feature transformation and nonlinear activation, and achieves state-of-the-art results on recommendation tasks.
Graph Attention Network \cite{velivckovic2017graph} leverages attention mechanisms in the neighbor aggregation process to improve the performance.

Our work differs from the above approaches, in that we develop a simple and effective GCN solution for a web-scale e-commerce embedding retrieval problem. To the best of our knowledge, we are the first to explore GCN's application to search embedding retrieval task. Accordingly, to make this happen, we have tried many techniques. In this paper, we will share our experience and present the best known approach.

% However, despite these improvements of GCN algorithms and their success in operating on large graph-structured data, no previous works have been done to apply GCN to e-commerce search engine setting where billions of queries and items are connected by user clicks. Here, we fill the gap and show GCN can be applied to e-commerce search engine vie graph embedding learning and retrieve more semantically relevant items to significantly improve users’ search experience.

% In terms of algorithm design, our work is most closely related to LightGCN algorithm \cite{he2020lightgcn}. LightGCN simplify the design of GCN to make it more concise and appropriate for collaborative filtering in recommendation task, where the node of uses and item graph are only described by a one-hot ID. LightGCN demonstrated that the feature transformation and non-linear activation function used in others GCN work \cite{????} will not contribute to learn better features when nodes has not rich attributes as input features. Similarly, the features used for semantic retrieval are few, see \ref{Features used for learning}. We fundamentally scale LightGCN to billions query-item graph learning by using pruned adjacent list to sample graph neighbors and further improve it's performance on semantically retrieve task by attention mechanisms and mask-technique.

\subsection{Embedding Retrieval in Search Engine}
Recently, embedding retrieval technologies have been widely adopted in the modern recommendation and advertising systems~\cite{youtube2016, mind2019, tree2018}, while have not been widely used in search engine yet. We find a few works about retrieval problems in search engine~\cite{palangi2016deep,vu2017search}, while they have not been applied to the industrial production system. DPSR~\cite{zhang2020towards} is one of the first practical explorations in this direction of applying embedding retrieval in the industrial search engine system. Moreover, the well known DSSM~\cite{Huang:2013:LDS:2541176.2505665} and its following work  CDSSM~\cite{Shen:2014:LSR:2567948.2577348} have pioneered the work of using deep neural networks for relevance scoring, which is very different task from embedding retrieval though.




% LightGCN...: when each node is only described by a one-hot ID, the feature transformation and non-linear activation function used in [?,?,?] will not contribute to learn better features.


% The leanable aggregation functions of GraphSAGE are: Mean aggregator, LSTM aggregator and Pooling aggregator. A number of follow-up work proposed variation of ,such as graph attention layer \cite{velivckovic2017graph}, importance pooling\cite{ying2018graph} and light graph convolution\cite{he2020lightgcn}.

% \begin{equation}
% H^{(l+1)} = \sigma(\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}H^{(l)}W^{(l)})
% \end{equation}

% Here, $\tilde{A} = A + I_{N}$ is the adjacency matrix, $I_{N}$ is the identity matrix and $\tilde{D} = \sum_{j} \tilde{A_{ij}}$. $\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}$ is the symmetrically normalized graph Laplacian, namely, the graph convolution martix. $H^{(l)} \in \mathbb{R}^{N \times D}$ is the representation in the l-th layer, and $H^(0) = X$. $W^{l}$ is the trainable parameters weight martix in layer $l$, which is used for feature transformation. $\sigma(\cdot)$ is the non-linear activation function, such as $ReLU(\cdot) = max(0, \cdot)$.



% \begin{equation}
% h_{\mathcal{N}_{(v)}}^{l+1} = \textsc{AGGREGATE}_{l}(\{ h_{\mathcal{N}_{(v)}}^{l}, \forall_{u} \in \mathcal{N}_{(v)} \});
% \end{equation}
% \begin{equation}
% h_{v}^{l+1} = \sigma \left( (\mathbf{W}^{l} \cdot \textsc{CONCAT}(h_{v}^{l}, h_{\mathcal{N}_{(v)}}^{l+1}) \right);
% \end{equation}

% Here, in $l-th$ layer, for each node $v \in \mathcal{V}$, the $\textsc{AGGREGATE}$ function aggregates the representations of nodes in its sampled neighborhood, $\{ h_{\mathcal{N}_{(v)}}^{l}, \forall_{u} \in \mathcal{N}_{(v)} \}$, into a single representation vector $h_{\mathcal{N}_{v}}^{l+1}$. $\mathcal{N}$ is a neighbor sampling function. Then GraphSAGE concatenates $h_{\mathcal{N}_{v}}^{l+1}$ with the node representation $h_{v}^{l}$ and feed them through a fully connected layer with nonlinear activation function $\sigma$, which generate new representations to be used at next layer, i.e., $h_{v}^{l+1}$, $v \in \mathcal{V}$.



==> 5-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we have proposed a GCN based approach for embedding retrieval in search engine. We also extensively study the offline comparison with other baseline models, and the results show that the proposed SearchGCN is both effective in retrieval quality metrics and training efficiency. Consequentially, we have successfully deployed SearchGCN to one of largest e-commerce search engine in the world, with significant business metric gains in the online A/B test.

